The Glass Ceiling of Automatic Evaluation in Natural Language Generation

Automatic evaluation metrics capable of replacing human judgments are critical to allowing fast development of new methods. Thus, numerous research efforts have focused on crafting such metrics. In this work, we take a step back and analyze recent progress by comparing the body of existing automatic metrics and human metrics altogether. As metrics are used based on how they rank systems, we compare metrics in the space of system rankings. Our extensive statistical analysis reveals surprising findings: automatic metrics -- old and new -- are much more similar to each other than to humans. Automatic metrics are not complementary and rank systems similarly. Strikingly, human metrics predict each other much better than the combination of all automatic metrics used to predict a human metric. It is surprising because human metrics are often designed to be independent, to capture different aspects of quality, e.g. content fidelity or readability. We provide a discussion of these findings and recommendations for future work in the field of evaluation.

==> 01_related_work.tex <==
\paragraph{Evaluation of evaluation metrics}
There has been various efforts to measure the levels of correlation between human judgments and existing metrics.

\paragraph{Ranking-based analysis}
 \citet{novikova-etal-2018-rankme} report that ``relative rankings yield more discriminative results than absolute assessments''
 
 \cite{peyrard-etal-2021-better} argued that it is better to aggregate system scores based on rankings instead of simply reported averages. The ranking aggregation is performed with the Bradley{--}Terry model.
 Item Response Theory (IRT) \cite{dras-2015-squibs} has been applied to perform dataset filtering \cite{lalor-etal-2016-building,lalor-etal-2019-learning}, evaluate chatbots from human assessments \cite{sedoc-ungar-2020-item}, and aggregate human assessments in machine translation \cite{dras-2015-squibs}.
 Since 2015, the Workshop on Machine Translation (WMT) has been using TrueSkill \cite{true_skill} , a variant of BT, to rank models based on human assessments following the methodology of \newcite{sakaguchi-etal-2014-efficient}.
 
 \cite{colombo2022} introduces Kemeny consensus, a ranking method to compare systems across tasks and datasets 

==> backup_.tex <==



\section{Ajouter les moyennes}
% ajouter les correlations metric entre metric automatics. 
% seuiller les arretes pour faire un truc jolie
% Nathan lire louvain pour le presenter + sortir les communauté 
% Seuiller les arretes. 
% Analyse avec les metrics importantes. 
% rajouter des belle heatmap + réduire les $\lamdba$ + résiduel cost
% defficulté intrinsic du pb 



\section{Conclusion \& Future Research directions}




\newpage


\section{Motivation}
For NLG evaluation, there are several types of human annotations and many automatic evaluation metrics crafted to approximate them. Often, researchers focus on comparing a single evaluation metric to human metrics with the goal of replacing the human metric with an automatic one. 

Typically, the comparison is done by computing some kind of correlation between human and automatic metrics based on the score they provide to systems' outputs on test sets.

Recently, several works have discussed the importance to think more about the ranking induced by the metric rather than the scores they output. 

In this work, we propose to take a step back and have a higher level view of the field: We compare the set of existing automatic evaluation metrics with the set of human metric. In particular, following recent recommendations, we perform these comparisons based on rankings rather than scores.



\subsection{RQ1}
Do the existing automatic metrics "explain" the human metrics? 
i.e., is it possible to replace the human metric with a combination of automatic ones? 

\textbf{Formally}: Linear decomposition after representing metrics with Borda counts

\subsection{RQ2}
Do automatic metrics have systematic bias, all modeling similar aspects of the problem leaving some dimensions of human evaluation aside? 
i.e., What is the similarity structure of metrics, projecting both automatic and evaluation ones together.

\textbf{Formally}: Define a similarity function between ranking and use to (i) visualize and (ii) analyze the general similarity structure.

\subsection{Questions}
\begin{enumerate}
    \item Is our set of metrics/dataset representative enough?
    \item Currently, the proposed solutions to RQ1 and 2 are purely quantitative, is it a problem? For example, if we notice that human metrics are different from automatic ones (there is a systematic bias in evaluation metrics), what are the dimension ignored by the field of automatic metrics?
    \item In general, what kind of claims would we like to see?
\end{enumerate}


\section{Ideas}
Given a human metric $M_h$ seen as a ground truth, one wishes to identfy the metric(s) that are clostest to $m_h$. Current methods rely on Kendall/Spearman correlation \cite{zhao2019moverscore,zhang2019bertscore,clark-etal-2019-sentence}. These papers say that among $M$ metrics $m_1, \ldots, m_M$, the best one is:
\[ m^* = \mathrm{argmax} \, \, K(m_i, m_h), \]
for a correlation function $K$. 

\medskip

\noindent Beware there exist several human metrics, for example for the Webnlg task (data2text \footnote{Given the following example of triple (see bellow):  \texttt{(John\_Blaha birthDate 1942\_08\_26) (John\_Blaha birthPlace San\_Antonio) (John\_E\_Blaha job Pilot)} the goal is to generate \texttt{John Blaha, born in San Antonio on 1942-08-26, worked as a pilot}.}) is evaluated by human annotators along four different axes: 
\begin{itemize}
    \item Data Coverage: Are all the description presented in the data included in the text? 
    \item Relevance: Does the text contains only predicates found in the data?
    \item Correctness: Are predicates found in the data correctly mentioned and adequately introduced? 
    \item Text structure: Is the produced text well-structured, grammatically correct and written in acceptable English?
    \item Fluency: Does the text progress naturally? Is it easy to understand? Is it a coherent whole?
\end{itemize}

\begin{remark}
We should switch utterance and system.
\end{remark}

\subsection{Question 0}
Data vizualisation en 2D. Multidimensionnal scaling (generalization of PCA). \url{https://www.stat.pitt.edu/sungkyu/course/2221Fall13/lec8_mds_combined.pdf} (induit sur les ranks). 



\subsection{First question}
 Maybe an interesting question: for a given human metric $m_h$ and quantitative metrics $m_1, \ldots, m_N$ what do compose the human metric $m_h$? How can we best explain $m_h$ with a reduced set of metrics from  $m_1, \ldots, m_N$ ?

To solve this problem master Noiry proposes to reduce this problem to a regression.
Denotes by $X_1=\begin{pmatrix}
 & m_1 & \cdots & m_N\\
u_1 &  & &  & \\
\cdots  &  & &  & \\\
u_n &  & &  & \ 
\end{pmatrix} \in \mathrm{R}^{n \times M} $ and $Y_1 =\begin{pmatrix}
m_h\\
\\
\\
\end{pmatrix}$  both contains the borda counts. Thus $X_1 a = \begin{pmatrix}
r_1^Ta \\
\cdots \\
r_n^Ta \\
\end{pmatrix} $
\begin{equation}
    \mathrm{min}_{a \in \mathrm{R}^n} \sum\limits_{i=1}^N ||X_i a - Y_i ||^2_2 + \lambda \Omega(a)
\end{equation}
where n is the number of instance labelled by each system, N is the number of metrics. We thus have a training set of $(X_i,Y_i)$ this can be used for either the systems or the utterances. 


\subsection{Second question: What metrics are most similar?}

We propose to do a clustering of metric based on the rank \url{https://indico.math.cnrs.fr/event/3002/attachments/1193/1312/Anna_Korba_IHES18.pdf} for the djoker. 

Find the different cluster $C_1,\cdots,C_k$ then do an aggregation.


\section{Analysis}



==> mds_analysis.tex <==

\section{MDS}

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/DIALOG_pcStauFalse.pdf}
         \caption{Dialog pc System}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/DIALOG_tcStauFalse.pdf}
         \caption{Dialog tc System}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/FLICKRStauFalse.pdf}
         \caption{Flickr System}
         \label{fig:five over x}
     \end{subfigure}
 \\
             \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/REAL_SUMStauFalse.pdf}
         \caption{Real Sum System}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/SUM_EVALStauFalse.pdf}
         \caption{SUM EVAL System}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/MLQEStauFalse.pdf}
         \caption{MLQE System}
         \label{fig:five over x}
     \end{subfigure}
 \\
             \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/TAC_08StauFalse.pdf}
         \caption{TAC 8 System}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/TAC_09StauFalse.pdf}
         \caption{TAC 9 System}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/TAC_11StauFalse.pdf}
         \caption{TAC 11 System}
         \label{fig:five over x}
     \end{subfigure}
     \caption{System Level}
\end{figure*}


\begin{figure*}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/DIALOG_tcTtauFalse.pdf}
         \caption{Dialog tc Text}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/FLICKRTtauFalse.pdf}
         \caption{Flickr Text}
         \label{fig:five over x}
     \end{subfigure}
 \\
             \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/REAL_SUMTtauFalse.pdf}
         \caption{Real Sum Text}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/SUM_EVALTtauFalse.pdf}
         \caption{SUM EVAL Text}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/MLQETtauTrue.pdf}
         \caption{MLQE Text}
         \label{fig:five over x}
     \end{subfigure}
 \\
             \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/TAC_08TtauTrue.pdf}
         \caption{TAC 8 Text}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/TAC_09TtauTrue.pdf}
         \caption{TAC 9 Text}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{all_mds/TAC_11TtauTrue.pdf}
         \caption{TAC 11 Text}
         \label{fig:five over x}
     \end{subfigure}
     \caption{Utterance Level}
\end{figure*}

